Improved Bounds for Scheduling Flows under Endpoint Capacity Constraints

We study flow scheduling under node capacity constraints. We are given capacitated nodes and an online sequence of jobs, each with a release time and a demand to be routed between two nodes. A schedule specifies which jobs are routed in each step, guaranteeing that the total demand on a node in any step is at most its capacity. A key metric in this scenario is response time: the time between a job's release and its completion. Prior work shows no un-augmented algorithm is competitive for average response time, and that a constant factor competitive ratio is achievable with augmentation exceeding 2 (Dinitz-Moseley Infocom 2020). For maximum response time, the best known result is a 2-competitive algorithm with a augmentation 4 (Jahanjou et al SPAA 2020). We improve these bounds under various response time objectives. We show that, without resource augmentation, the best competitive ratio for maximum response time is $\Omega(n)$, where $n$ is the number of nodes. Our Proportional Allocation algorithm uses $(1+\varepsilon)$ resource augmentation to achieve a $(1/\varepsilon)$-competitive ratio in the setting with general demands and capacities, and splittable jobs. Our Batch Decomposition algorithm is $2$-competitive (resp., optimal) for maximum response time using resource augmentation 2 (resp., 4) in the setting with unit demands and capacities, and unsplittable jobs. We also derive bounds for the simultaneous approximation of average and maximum response time metrics.

==> l_p.tex <==

%p-norm stuff from Dinitz Moseley 
For optimizing p-norm metric, we consider a slight modification of Linear Programming relaxation formulation given by Dinitz-Moseley \cite{dinitz+moseley.reconfigurable.20}. Let $S$ denote the set of all requests. Let $S_w = \{j\in S: |\{u_j, v_j\} \cap \{w\}|= 1\}$ denote the set of all requests adjacent to node $w$. We first prove that this is a valid linear programming relaxation, and then we will show that the same dual fitting argument given by Dinitz-Moseley works for optimizing p-norm metric for all finite $p \geq 1$. 

\begin{center}
    \begin{align*}
    \min & \sum_{j\in S}\sum_{t\geq r_j} (t-r_j)^p x_{j,t}&  \\
    \mbox{s.t. }\ & {\sum_{t\geq r_j} x_{j,t} \geq 1},   && \forall j \in S
    \\
    &\sum_{j\in S_w} x_{j,t} \leq 1 &&\forall w \in S, t \in \mathbb{N}
    \\
    &x_{j,t} \ge 0 &&\forall j\in S, t\in \mathbb{N}
    \end{align*}
\end{center}

\begin{lemma}
If there is a schedule with sum of the $p^{th}$power of flow times at most $F$, then there is a solution to the LP of cost at most $F$.
\end{lemma}

\begin{proof}
Consider a schedule with sum of the $p^{th}$ power of flow times at most $F$. We create an LP solution as follows: if job $i$ is scheduled at time $t$, then we set $x_{j,t} = 1$, otherwise we set $x_{j,t} = 0$. Each request is served, so the first LP constraint is satisfied. Moreover, since Since this is a feasible schedule, the requests in each round of the schedule form a matching, which implies that the second constraint is satisfied. Thus, this is a feasible LP solution. Since the $p^{th}$ power of a request's flow times $i$ is 
$\sum_{t \geq r_j}(t - r_j)^p x_{j,t}$, the sum $p^{th}$ power of all requests is the objective value of the LP solution. 
\end{proof}

The dual of Linear Programming relaxation formulation is the following. 
\begin{center}
    \begin{align*}
    \max & \sum_{j\in S} \alpha_j - \sum_{u\in V}\sum_{t \in \mathbb{N}}\beta_{u, t} \\
    \mbox{s.t. }\ & { \alpha_j - \beta_{u_j, t}  - \beta_{v_j, t}  \leq (t-r_j)^p},   && \forall j \in S, t \in \mathbb{N}
    \\
    & \alpha_j \geq 0 && \forall i \in S
    \\
    &\beta_{j,t} \ge 0 &&\forall j\in S, t\in \mathbb{N}
    \end{align*}
\end{center}

Let $G(t)$ be the (multi)graph of all pending requests at time $t$, and let $d_v(t)$ the number of requests on node $v$ in $G(t)$. We show that the following values of the dual variable gives a feasible solution. For every $i \in S$, 
\begin{equation*}
    \begin{split}
    \alpha_j &= \frac{d_{u_j}(r_j)+d_{v_i}(r_j)}{2(2+k)}\\
    \beta_{u_j, t} &= \frac{d_u(t)}{2(2+k)}
    \end{split}
\end{equation*}

\begin{lemma}
\label{thm: Dinitz_Moseley_unit}
 $\alpha_j - \beta_{{u_j}, t}  - \beta_{{v_i}, t}  \leq t-r_j, \forall i \in S, t \in \mathbb{N}$
\end{lemma}

\begin{lemma}
$\alpha_j - \beta_{{u_j}, t}  - \beta_{{v_i}, t}  \leq (t-r_j)^p, \forall i \in S, t \in \mathbb{N}$
\end{lemma}

\begin{proof}
From lemma \rom{4.2} of Dinitz-Moseley \cite{dinitz+moseley.reconfigurable.20}, for all $i \in S$ and  $t \in \mathbb{N}$, we have that $\alpha_j - \beta_{{u_j}, t}  - \beta_{{v_i}, t}  \leq t-r_j$.  Since $t-r_j \in \mathbb{N} \cup \{0\}$, it follows that $t-r_j \leq (t-r_j)^p$ for all finite $p \geq 1$. Hence, $\alpha_j - \beta_{{u_j}, t}  - \beta_{{v_i}, t}  \leq (t-r_j)^p, \forall i \in S, t \in \mathbb{N}$
\end{proof}


\begin{lemma}
For optimizing any p-norm metric, with a resource augmentation of a factor of $(2+k)$ where $k \in \mathbb{N} \leq 2$, FIFO Maximal Matching is $2(2+k)/k-$ competitive. 
\label{thm:FIFO_p_norm}
\end{lemma}

\begin{proof}
This proof is the same as the proof given by Dinitz-Moseley in section 4 of Dinitz-Moseley \cite{dinitz+moseley.reconfigurable.20}. 
\end{proof}

\begin{theorem}
FIFO, with a resource augmentation factor of $(2+k)$ where $k =\{1, 2\}$, achieves $2/k-$ competitive under the maximum response time metric, and achieves $2(2+k)/k-$ competitive
for all $p-$norm where $p \geq 1$. 
\label{thm: unit_all_norm}
\end{theorem}

\begin{proof}
It follows immediately from lemma \ref{thm:FIFO_p_norm} and lemma \ref{thm:FIFO_upperbounds}. 
\end{proof}

==> makespan.tex <==
\section{Offline \texorpdfstring{$(1 + o(1))$}{}-Approximation for Makespan}
Consider the following linear program forumation, parameterized by $C$.

\begin{align}
\sum_{t = a\sqrt{C}+1}^{(a+1)\sqrt{C}} \ \sum_{j \ni i} d_j x_{j,t} &\le c_i \sqrt{C} &&\forall i \in P, a \in \mathbb{N} \label{LP:makespan:pack}
\\
\sum_{r_j = t}^C x_{j,t} &\ge 1 &&\forall j \in J \label{LP:makespan:cover}
\end{align}

\begin{lemma}
For any schedule with makespan $C$ there exists a solution to the LP parameterized by $C$. 
\end{lemma}

\begin{proof}
Consider any valid schedule  with makespan $C$. For each request $j$, set $x_{j,t} \leftarrow 1$ if $j$ is scheduled in round $t$, and set to $0$ otherwise. By the validity of the schedule, all jobs are scheduled, so contraint (\ref{LP:makespan:cover}) is satisfied. For constraint (\ref{LP:makespan:pack}), consider any port $i$ and interval $[a\sqrt{C} + 1, (a+1)\sqrt{C}]$ where $a \in \mathbb{N}$. By the validity of the schedule, there is at most one request scheduled on $i$ in every round in the interval. So the sum of the demands of all requests scheduled in the interval is no more than $c_i \sqrt{C}$. Therefore, constraint (\ref{LP:makespan:pack}) is satisfied.
\end{proof}


\begin{lemma}[Theorem 3 in \cite{karp+leighton+rivest.globalwire.83}]
    Let $\mathbf{A}$ be a real-valued $r \times s$ matrix, let $\mathbf{x}$ be a real-valued $s$-vector, let $\mathbf{b}$ be a real-valued $r$-vector such that $\mathbf{Ax} = \mathbf{b}$, and let $\Delta$ be a positive real number such that in every column of $\mathbf{A}$ we have 
    \begin{enumerate*}[label=(\alph*)]
        \item the sum of the positive elements is at most $\Delta$ and
        \label{rounding:pos}
        \item the sum of the negative elements is at least $- \Delta$.
        \label{rounding:neg}
    \end{enumerate*}
    Then we can compute an integral $s$-vector $\mathbf{\hat{x}}$ such that
    \begin{enumerate*}[label=(\roman*)]
        \item for all $k$, $1 \le k \le s$, either $\mathbf{\hat{x}}_k = \lfloor \mathbf{x}_k \rfloor$ or $\mathbf{\hat{x}}_k = \lceil \mathbf{x}_k \rceil$, and
        \label{rounding:integral}
        \item $\mathbf{A\hat{x}} = \mathbf{\hat{b}}$, where $\mathbf{\hat{b}}_k - \mathbf{b}_k < \Delta$ for $1 \le k \le r$. 
        \label{rounding:difference}
    \end{enumerate*}
    In the case that all entries in $\mathbf{A}$ are integers, then a stronger bound applies: $\mathbf{\hat{b}}_k - \lceil \mathbf{b}_k \rceil \le \Delta - 1$ for $1 \le k \le r$.
\label{lem:klr.rounding}
\end{lemma}

\begin{lemma}

\end{lemma}

\begin{algorithm}
find a variable assignment $\{x\}_{j,t}$ that satisfies constraints (\ref{LP:makespan:pack}) and (\ref{LP:makespan:cover}) for minimum $C$ \;
apply Lemma \ref{lem:klr.rounding} to derive an integral solution\;
\caption{Makespan Minimization}
\end{algorithm}

